Global Reinforcement Learning: Beyond Linear and Convex Rewards via Submodular Semi-gradient Methods

In classic Reinforcement Learning (RL), the agent maximizes an additive objective of the visited states, e.g., a value function. Unfortunately, objectives of this type cannot model many real-world applications such as experiment design, exploration, imitation learning, and risk-averse RL to name a few. This is due to the fact that additive objectives disregard interactions between states that are crucial for certain tasks. To tackle this problem, we introduce Global RL (GRL), where rewards are globally defined over trajectories instead of locally over states. Global rewards can capture negative interactions among states, e.g., in exploration, via submodularity, positive interactions, e.g., synergetic effects, via supermodularity, while mixed interactions via combinations of them. By exploiting ideas from submodular optimization, we propose a novel algorithmic scheme that converts any GRL problem to a sequence of classic RL problems and solves it efficiently with curvature-dependent approximation guarantees. We also provide hardness of approximation results and empirically demonstrate the effectiveness of our method on several GRL instances.

==> sections/extended_related_works.tex <==
\mypar{General Utilities and Convex \RL} As already depicted in section \ref{sec:general_utilities}, General Utilities RL (GURL) aims to find a policy that optimizes a functional of state(-action) visitation distributions. In the case of convex (concave) functionals, this framework is often called Convex (Concave) Utilities RL and it has found applications in a multitude of areas, including exploration \cite{mutti2022importance} and experimental design \cite{Hazan2019, Zahavy2021,Duff2002, Tarbouriech2019, tarbouriech2020active,Mutny2023}. \citeauthor{mutti2022challenging} has recently shown that Convex RL is fundamentally ill-posed as it optimizes the performance of expected state(-action) distributions rather than of empirical state(-action) distribution that can actually be induced by the agent interacting with the environment. When the problem is properly captured convexity is lost \cite{mutti2022challenging}. In this work we argue that by adopting a combinatorial optimization perspective we can exploit useful structural properties for this practical problem setting, namely submodularity, supermodularity, and suBmodularity-suPermodularity. Moreover, through this change of perspective, from convex to combinatorial optimization, we managed to make a first step towards building efficient approximate algorithms for this hard problem, which is currently considered an open problem \cite{mutti2022importance}.

\mypar{Beyond Markovian \RL}
%We extend the modelling ability of classical reinforcement learning with Markov chain and Markovian rewards and consider a class of non-Markovian reward functions. 
Several prior works in \RL identify the deficiency in the modelling ability of classical Markovian rewards. This manifests itself especially when exploration is desired, e.g., when the transition dynamics are not completely known \cite{Tarbouriech2019, Hazan2019} or when the reward is not completely known \cite{lindner2021information, Belogolovsky2021}. While all these works deal with the shortcomings of Markovian rewards they have two fundamental differences from this work. First, they face the problem from the lenses of a specific application rather than from a general mathematical perspective leading to problem-independent structural assumptions as we do in this work. Second, they do not approach the problem from a combinatorial viewpoint as we do, despite its inherent combinatorial nature, as shown in this work. Another stream of works tackles the problem of non-Markovian rewards from the angle of automata theory, studying certain classes of rewards from the perspective of logic and formal language theory \cite{gaon2020reinforcement, de2013linear, brafman2018ltlf}. The analysis within these works are orthogonal to ours. Nonetheless, it would be particularly interesting to understand how the mathematical structures we propose are related with the logic assumptions typically made in these works, and whether solution methods can be transferred between these different problem specifications. To the best of our knowledge, the closest work to ours is \citep{prajapat2023submodular}, which considers non-Markovian rewards with a submodular structure. Beyond being limited to the submodular case, this work does not suggest an algorithmic scheme based on the combinatorial optimization viewpoint we have introduced, and proposes to solve the problem via a policy gradient method.

\mypar{Submodular, Supermodular, and suBmodular-suPermodular Function Maximization}
Submodular and supermodular functions have been vastly studies in the field of combinatorial optimization.
While submodular functions have found many applications in machine learning \citep{krause2014submodular,bilmes2022submodularity,tohidi20}, supermodular functions have been mostly applied in game theory, economics, and decision theory \citep{amir2005supermodularity, chambers2009supermodularity}.
Historically, submodular and supermodular function maximization have been treated with significantly different approaches \citep{krause2014submodular, iwata2008submodular}. Recently, new optimization methods based on discrete semidifferentials have been developed \cite{iyer2013fast, iyer2015polyhedral}. 
These methods, based on the optimization of modular lower bounds, make it possible to treat submodular and supermodular function maximization in a unified manner. More recently, this approach has been extended to the case of BP function maximization \citep{bai2018greed}. While in the fully-curved setting the problem has been shown to be inapproximable to any factor, in the bounded-curvature case the problem has also been studied under cardinality and matroid constraints, where there exist efficient algorithms achieving an approximation ratio of $\nicefrac{1}{k_Q}[1-e^{{-(1-k^G)k_Q}}]$ for cardinality constraint, and $\nicefrac{1-k^G}{(1-k^G)k_Q + p}$ for $p \geq 1$ matroid constraints. We extend these results by studying the possibilities and limitations of these structural assumptions in the context of CMPs introducing a novel type of constraint, namely the CMP constraint. 

While submodularity has been vastly explored in the context of sequential decision making under uncertainty \citep{yue2011linear, takemori2020submodular, gabillon2013adaptive}, only a recent work considers supermodular and BP structural assumptions \citep{narang2022interactive}. Moreover, we believe that ours is the first work that exploits supermodularity in the context of RL and attributes to it a meaningful semantic interpretation. 

==> v_line_patch.tex <==
\errorcontextlines\maxdimen

% begin vertical rule patch for algorithmicx (http://tex.stackexchange.com/questions/144840/vertical-loop-block-lines-in-algorithmicx-with-noend-option)
\makeatletter

\newcommand*{\algrule}[1][\algorithmicindent]{\makebox[#1][l]{\hspace*{.5em}\vrule height .7\baselineskip depth .3\baselineskip}}%

\newcount\ALG@printindent@tempcnta
\def\ALG@printindent{%
    \ifnum \theALG@nested>0% is there anything to print
        \ifx\ALG@text\ALG@x@notext% is this an end group without any text?
            % do nothing
            \addvspace{-3pt}% FUDGE for cases where no text is shown, to make the rules line up
        \else
            \unskip
            % draw a rule for each indent level
            \ALG@printindent@tempcnta=1
            \loop
                \algrule[\csname ALG@ind@\the\ALG@printindent@tempcnta\endcsname]%
                \advance \ALG@printindent@tempcnta 1
            \ifnum \ALG@printindent@tempcnta<\numexpr\theALG@nested+1\relax% can't do <=, so add one to RHS and use < instead
            \repeat
        \fi
    \fi
    }%
\usepackage{etoolbox}
% the following line injects our new indent handling code in place of the default spacing
\patchcmd{\ALG@doentity}{\noindent\hskip\ALG@tlm}{\ALG@printindent}{}{\errmessage{failed to patch}}
\makeatother
% end vertical rule patch for algorithmicx
